The temperature of the diffuse HI in the Milky Way II: Gaussian decomposition of the HI 21 cm absorption spectra

We discuss physical conditions in Galactic neutral hydrogen based on deep, high velocity resolution interferometric HI 21 cm absorption spectroscopy towards 33 compact extra-galactic radio sources. The HI 21 cm optical depth spectra have root-mean-square noise values \lesssim 10^{-3} per 1 km/s velocity channel, i.e., sufficiently sensitive to detect HI 21 cm absorption by the warm neutral medium (WNM). Comparing these spectra with HI 21 cm emission spectra from the Leiden-Argentine-Bonn (LAB) survey, we show that some of the absorption detected on most sightlines must arise in gas with temperatures higher than that in the stable cold neutral medium (CNM). A multi-Gaussian decomposition of 30 of the HI 21 cm absorption spectra yielded very few components with line widths in the temperature range of stable WNM, with no such WNM components detected for sixteen of the thirty sightlines. We find that some of the detected HI 21 cm absorption along thirteen of these sightlines must arise in gas with spin temperatures larger than the CNM range. For these sightlines, we use very conservative estimates of the CNM spin temperature and the non-thermal broadening to derive strict upper limits to the gas column densities in the CNM and WNM phases. Comparing these upper limits to the total HI column density, we find that typically at least 28% of the gas must have temperatures in the thermally unstable range (200-5000 K). Our observations hence robustly indicate that a significant fraction of the gas in the Galactic interstellar medium has temperatures outside the ranges expected for thermally stable gas in two-phase models.

==> readme <==
%auto-ignore

This file contain information regarding the paper "The temperature of the diffuse HI in the Milky Way II: Gaussian decomposition of the HI 21 cm absorption spectra"

Authors: Nirupam Roy, Nissim Kanekar and Jayaram N. Chengalur 

Comments: 18 pages, 8 figures. Accepted for publication in MNRAS. The definitive version will be available at http://mnras.oxfordjournals.org/

The contact details of the first author are as follows
Nirupam Roy
email  : nirupam@mpifr-bonn.mpg.de
Address: Max-Planck-Institut fur Radioastronomie,
         Auf dem Hugel 69, D-53121 Bonn, Germany
Tel    : +49 228 525491

Abstract: We discuss physical conditions in Galactic neutral hydrogen based on deep, high velocity resolution interferometric HI 21 cm absorption spectroscopy towards 33 compact extra-galactic radio sources. The HI 21 cm optical depth spectra have root-mean-square noise values \lesssim 10^{-3} per 1 km/s velocity channel, i.e., sufficiently sensitive to detect HI 21 cm absorption by the warm neutral medium (WNM). Comparing these spectra with HI 21 cm emission spectra from the Leiden-Argentine-Bonn (LAB) survey, we show that some of the absorption detected on most sightlines must arise in gas with temperatures higher than that in the stable cold neutral medium (CNM). A multi-Gaussian decomposition of 30 of the HI 21 cm absorption spectra yielded very few components with line widths in the temperature range of stable WNM, with no such WNM components detected for sixteen of the thirty sightlines. We find that some of the detected HI 21 cm absorption along thirteen of these sightlines must arise in gas with spin temperatures larger than the CNM range. For these sightlines, we use very conservative estimates of the CNM spin temperature and the non-thermal broadening to derive strict upper limits to the gas column densities in the CNM and WNM phases. Comparing these upper limits to the total HI column density, we find that typically at least 28% of the gas must have temperatures in the thermally unstable range (200-5000 K). Our observations hence robustly indicate that a significant fraction of the gas in the Galactic interstellar medium has temperatures outside the ranges expected for thermally stable gas in two-phase models.

